Towards an Effective Decision Procedure for LTL formulas with Constraints

This paper presents an ongoing work that is part of a more wide-ranging project whose final scope is to define a method to validate LTL formulas w.r.t. a program written in the timed concurrent constraint language tccp, which is a logic concurrent constraint language based on the concurrent constraint paradigm of Saraswat. Some inherent notions to tccp processes are non-determinism, dealing with partial information in states and the monotonic evolution of the information. In order to check an LTL property for a process, our approach is based on the abstract diagnosis technique. The concluding step of this technique needs to check the validity of an LTL formula (with constraints) in an effective way. In this paper, we present a decision method for the validity of temporal logic formulas (with constraints) built by our abstract diagnosis technique.

==> CompGIBUFixBehaTCCP-macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                          %
%   LaTeX&packages setup   %
%                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\@ifundefined{mathindent}{\typeout{NO fleqn}}{\setlength{\mathindent}{.5\parindent}}
\@ifundefined{multicolsep}{\typeout{NO multicolsep}}{\setlength{\multicolsep}{1ex}}
\@ifundefined{columnseprule}{\typeout{NO columnseprule}}{\setlength{\columnseprule}{0.4pt}}
\makeatother

%%%%%%%%%%%%%%%%
%              %
% LOCAL MACROS %
%              %
%%%%%%%%%%%%%%%%

\newcommand*{\replicate}[1]{#1 \mathrel{\cdots} #1 \mathrel{\cdots}}

\makeatletter
\newenvironment{refresult}[1]%
{\Thm@shape@PlainIt@in{\smartref{#1}.}}
{\Thm@shape@PlainIt@out}
\makeatother

\newsmartprefix{rule}{Rule}
\newsmartsprefix{rule}{Rules}

\newcommand*{\closed}[1][A]{\ifempty{#1}{S}{s}elf-sufficient}

%constraint system of examples
\newcommand*{\CSex}{\mathbf{L}} 
\newcommand*{\CSexdom}{\mathcal{L}} 

%%DOMINI E ORDINAMENTI%%


%Sequenze chiuse per prefisso

\newcommand*{\Rr}{\mathbb{P}}%dominio sequenze reattive condizionali
\newcommand*{\leqRr}{\subseteq}
\monobioperator{\lubRr}{\cup}{\bigcup}
\monobioperator{\glbRr}{\cap}{\bigcap}
\newcommand*{\botRr}{\{\ecrs\}}
\newcommand*{\topRr}{\mathbf{CT}}

\newcommand*{\latticeRr}{\lattice{\Rr}{\leqRr}{\lubRr{}{}}{\glbRr{}{}}{\topRr}{\botRr}}
\newcommand*{\cpoRr}{\cpo{\Rr}{\leqRr}}
\newcommand*{\maxim}{\parensmathoper{maximal}}%op sequenze massimali
\newcommand*{\pat}{\parensmathoper{path}}%op percorsi
\newcommand*{\pref}{\leq_{\mathit{pref}}}%relazione prefissi

%Alberi

\newcommand*{\tree}{\parensmathoper{tree}}%op alberi
\newcommand*{\Tree}{\mathbb{T}}%dominio alberi
\newcommand*{\ordTree}{\unlhd}
% \newcommand*{\cpoTree}{\Fbox{$\cpo{\Tree}{\leqTree}$}}
% \newcommand*{\emptyTree}{\Fbox{$\Box$}}

%%INPUT-OUTPUT%%

\newcommand*{\alIO}{\parensmathoper{\alpha_{\mathit{io}}}}
\newcommand*{\gaIO}{\parensmathoper{\gamma_{\mathit{io}}}}

\newcommand*{\tfin}{\parensmathoper{\mathit{fin}}}
\newcommand*{\tinf}{\parensmathoper{\mathit{inf}}}
\newcommand*{\tmode}{\parensmathoper{\mathit{mode}}}

\newcommand*{\latticeIO}{\lattice{\IOdom}{\leqIO}{\lubIO{}{}}{\glbIO{}{}}{\topIO}{\botIO}}
\newcommand*{\cpoIO}{\cpo{\IOdom}{\leqIO}}
\newcommand*{\leqIO}{\subseteq}
\newcommand*{\IOdom}{\mathbb{IO}}
\monobioperator{\glbIO}{\cap}{\bigcap}
\monobioperator{\lubIO}{\cup}{\bigcup}
\newcommand*{\botIO}{\emptyset}
\newcommand*{\topIO}{\mathbf{IO}}

\newcommand*{\IODd}[2]{\Tp[\mathit{io}]{#1}{#2}}
\newcommand*{\IOF}{\F[\mathit{io}]}
\newcommand*{\IO}[2]{\pair{#1}{#2}}
\newcommand*{\BehaEqIO}{\BehaEq[\mathit{io}]}
\newcommand*{\BehaFinQIO}{\BehaFinQ[\mathit{io}]}
% \newcommand*{\BehaG}[2]{\syntaxoper{\GabbriObsSym}{#2}{#1}}
\newcommand*{\BehaIO}{\Beha[\mathit{io}]}
\newcommand*{\BehaQG}[3]{\syntaxoperEXT{#2}{\GabbriObsSym}{\Q{#2}{#3}}{#1}}%\BehaG{#1}{\Q{#2}{#3}}
\newcommand*{\BehaQIO}{\BehaQ[\mathit{io}]}

\newcommand*{\GabbriObsSym}{\mathcal{O}^{\mathit{io}}}
\newcommand*{\GabbriObs}{\parensmathoper{\GabbriObsSym}}

%%SEQUENZE FINITE%%

\newcommand*{\FIOdom}{\IOdom_{F}}
\newcommand*{\cpoFIO}{\cpo{\FIOdom}{\leqIO}}
\newcommand*{\projFinIO}{\parensmathoper{\pi_{\mathit{F}}}}%^{\IOdom}

\newcommand*{\projFinM}{\parensmathoper{\pi^{\C}_{\mathit{F}}}}
\newcommand*{\FM}{{\C[]}_{F}}
\newcommand*{\cpoFM}{\cpo{\FM}{\leqC}}


==> macro-desc-general.tex <==

\section{wgmacros-support.tex}

\macroTwOp{\BBrackets}
\macroTwOp{\Braces}
\macroTw{\extraArg}
\macroTw{\extraArgSc} 

\macroTw{\parensmathoper}
\macroTh{\syntaxoper}
\macroFo{\syntaxoperEXT}


\section{Abstract Interpretation \& Domains (wgmacros-absint)}

\macroSi{\lattice}
\macroOn{\al}
\macroOn{\ga}

\subsection{Default Concrete Domain (for paper body, to be localized)}

\macroREDEFz{\lubCbigsym}
\macroREDEFz{\glbCbigsym}
\macroREDEFz{\lubCsym}
\macroREDEFz{\glbCsym}

\macroZ{\C}
\macroZ{\leqC}
\macroZ{\geqC}
\macroZ{\nleqC}
\macroTw{\lubC}
\macroTw{\glbC}
\macroZ{\botC}
\macroZ{\topC}

\macroZ{\cpoC}
\macroZ{\latticeC}

\subsection{Default Concrete Domain (for paper body, to be localized)}

\macroREDEFz{\lubAbigsym}
\macroREDEFz{\glbAbigsym}
\macroREDEFz{\lubAsym}
\macroREDEFz{\glbAsym}

\macroZ{\A}
\macroZ{\leqA}
\macroZ{\nleqA}
\macroTw{\lubA}
\macroTw{\glbA}
\macroZ{\botA}
\macroZ{\topA}

\macroZ{\cpoA}
\macroZ{\latticeA}

\subsection{Generic Concrete Domain (for preliminaries)}

\macroZ{\CC}
\macroZ{\leqCC}
\macroZ{\nleqCC}
\macroTw{\lubCC}
\macroTw{\glbCC}
\macroZ{\botCC}
\macroZ{\topCC}

\macroZ{\cpoCC}
\macroZ{\latticeCC}

\subsection{Generic Abstract Domain (for preliminaries)}

\macroZ{\AA}
\macroZ{\leqAA}
(compare with $\not\leqAA$) \macroZ{\nleqAA} 
\macroTw{\lubAA}
\macroTw{\glbAA}
\macroZ{\botAA}
\macroZ{\topAA}

\macroZ{\cpoAA}
\macroZ{\latticeAA}

\subsection{Names/Notations of Standard Domains}

% still to be organized

\subsubsection{$\POS$}

\macroZ{\POS}
\macroTwOp{\POSpreabs}
\macroOn{\POSabs}
\macroOn{\POSconc}

\subsubsection{$\depthk$}

\macroOnOp{\depthk}
\macroOnOp{\KTerms}
\macroOnOp{\KCTerms}
\macroZ{\KVsyms}
\macroTw{\Kcut}
\macroTw{\KTp}
\macroTh{\Keval}
\macroZ{\KSz}

\section{Semantics (concrete/abstract)}

\subsection{DOMAINS and orders}

\macroTw{\cpo}

\macroOnOp{\interpC}
\macroOnOp{\interpA}
\macroZ{\leqIc}
\macroZ{\leqIa}
\macroZ{\nleqIc}
\macroZ{\nleqIa}

\subsection{TERMS (signature, positions, \ldots) }

\macroREDEFon{\mathT}
\macroREDEFz{\TermsSym}
\macroREDEFz{\LinTermsSym}

\macroZ{\Fsyms}
\macroZ{\Csyms}
\macroZ{\Dsyms}
\macroZ{\Vsyms}
\macroZ{\Psyms}

\macroTw{\SigTerms}
\macroOnOp{\Terms}
\macroOnOp{\CTerms}

\macroTw{\LinSigTerms}
\macroOnOp{\LinTerms}
\macroOnOp{\LinCTerms}

\macroZ{\leqT}

% \macroTwOp{\pos}
% \macroZ{\leqP}
\macroZ{\append}
\macroTh{\replace}
\macroZ{\rootPos}
\macroTw{\subterm}

\macroOn{\vars}
\macroZ{\fresh}

\macroTw{\termres}

\macroFoOp{\mgc}
\macroTh{\call}

\macroTw{\genrule}
\macroTh{\prule}
\macroFoOp{\mgrule}
\macroThOp{\mghead}

% \macroTw{\letop}

\macroZ{\Substs}
\macroZ{\CSubsts}
\macroOnOp{\MGC}
\macroREDEFz{\MGCsym}

\macroZ{\leqS}
\macroZ{\eqS}
\macroZ{\neqS}
\macroZ{\gtS}
\macroZ{\lubS}

\macroZ{\emptysubst}
\macroOn{\dom}
\macroOn{\range}
\macroOn{\img}
% \macroTw{\domrestriction}
\macroTw{\restrict}
\macroTw{\restrictVars}


\macroREDEFz{\ProgsSym}
\macroOnOp{\Progs}

\macroREDEFz{\ProgSym}
\macroOnOp{\prog}
\macroOnOp{\P}

\subsection{REWRITING AND NARROWING}

% \macroTw{\rewrule}

\macroOnOp{\rewrites}
\macroOnOp{\rewritesTo}
\macroTwOp{\rewriteStep}
\macroZ{\nrewrites}

\macroTwOp{\narrows}
\macroTwOp{\narrowsTo}
\macroThOp{\narrowStep}
\macroZ{\nnarrows}

\subsection{SEMANTICS INTERPRETATION FUNCTIONS}

\macroREDEFon{\mathC}
\macroREDEFz{\BehaSym}
\macroREDEFz{\SemSym}
\macroREDEFz{\TrSym}
\macroREDEFz{\OsemSym}
\macroREDEFz{\FSym}
\macroREDEFz{\TpSym}
\macroREDEFz{\evalSym}

\macroTw{\Q}
\macroTwOp{\Beha}
\macroTwOp{\Sem}
\macroThOp{\Tr}

\macroOn{\Osem}
\macroTwOp{\F}
\macroThOp{\Tp}
\macroThOp{\TpN}
\macroFoOp{\eval}
\macroThOp{\evalrules}

\macroZ{\FUNeq}

\macroOnOp{\I}
\macroOnOp{\Sz}
\macroOnOp{\Rz}

\subsection{PROGRAM EQUIVALENCES}

\macroThOp{\ProgEquiv}
\macroThOp{\BehaEq}
\macroThOp{\SemEq}

\subsection{PROOF TREES}

\macroFoOp{\sequent} Use \verb|\and| and \verb|\ands| within, \eg\
\verb|\sequent{a\and b \and c}{d}{e\\f}| or \verb|\sequent{a\ands b}{c}{d}| 
\begin{align*}
    &\sequent{a\and b \and c}{d}{e\\f} & & \sequent{a\ands b}{c}{d}
\end{align*}
% \macroFiOp{\twsequent}
% \macroFiOp{\manysequent}
% \macroSiOp{\thsequent}

\subsection{TREES}

\macroOn{\Theight}
\macroOn{\Theight*}
\macroTw{\Tnode}
\macroOn{\Tpaths}
\macroOn{\Tmaxpaths}
\macroOn{\Troot}
\macroOn{\Tsiblings}
\macroOn{\Tsons}
\macroFo{\Tstep}
\macroOn{\Tsteps}
\macroTw{\Tsubterm}

\subsection{Miscellaneous}

\macroZ{\glb}
\macroZ{\lub}
\macroOn{\mgu}

\macroOnOp{\lfp}
\macroTwOp{\lfpof}
\macroTw{\iter}
\macroTh{\sameof}

\macroOnOp{\gfp}
\macroTwOp{\gfpof}
\macroTw{\downiter}

\macroOn{\len}
\macroOn{\prefixtree}
\macroTw{\equivClass}


\section{wgmacros-math.tex}


\macroZ{\implies}
\macroZ{\nimplies}

\macroTw{\set}
\macroTw{\set*}

\macroTw{\mset}
\macroTw{\mset*}

\macroZ{\dfn}
\macroZ{\revdfn}

\macroTwOp{\zseq}
\macroTwOp{\seq}

\macroZ{\coloneqq}
\macroZ{\coloneq}
\macroZ{\eqqcolon}

\macroOn{\mathoper}

\macroTw{\pair}
\macroTh{\triple}
\macroFo{\quadruple}

\macroZ{\true}
\macroZ{\false}
\macroOnOp{\id}
\macroZ{\True}
\macroZ{\False}

% Negated symbols

(compare with $\not\in$) \macroZ{\nin}

\macroZ{\ngg} 
\macroZ{\notin}
\macroZ{\npreccurlyeq}
\macroZ{\nrightarrowtriangle}
\macroZ{\nsimeq}
\macroZ{\nsqsubseteq}
\macroZ{\nRightarrow}


\macroZ{\powerset}
\macroZ{\llbracket}
\macroZ{\rrbracket}

\section{wgmacros-misc.tex}

% \macroOn{\mlst} 
\texttt{\string\mlst\{\}} $\rightarrow$ $\mlst{}$\interfill
\texttt{\string\mlst\{a\#b\}} $\rightarrow$ $\mlst{a#b}$\intrasep

\txmacroZ{\currenttime}
\macroOn{\mathscr} 

\txmacroZ{\eg}
\txmacroZ{\etc}
\txmacroZ{\ie}  
\txmacroZ{\resp}
\txmacroZ{\st}  
\txmacroZ{\wrt} 
\txmacroZ{\wlg} 

\txmacroOnOp{\paradigm}
\txmacroZ{\proglang}
\txmacroOnOp{\program}
\txmacroOnOp{\programs}
\txmacroZ{\progequiv}
\txmacroZ{\progequivs}
\txmacroZ{\progrule}
\txmacroZ{\progrules}
\txmacroOnOp{\query}
\txmacroOnOp{\queries}
\txmacroOnOp{\expression}
\txmacroOnOp{\expressions}
\txmacroOnOp{\deffun}
\txmacroOnOp{\deffuns}


\txmacroTw{\bibURLext}
\txmacroOn{\bibURL}
\txmacroTw{\href}

\txmacroOn{\email}

\txmacroOn{\xcite}

\txmacroOn{\Fbox}
\txmacroOn{\Flbox}
% 
% With draft off
% \texttt{\string\Dbox\{aa\}} $\rightarrow$ $\Dbox{aa}$\intrasep
% With draft on
% \texttt{\string\Dbox\{aa\}} $\rightarrow$ $\Dbox{aa}$\intrasep
% \macroOn{}


==> macro-desc-support.tex <==
\usepackage[nodate]{datetime}
\usepackage{babel}
\usepackage{amsmath}
\usepackage{amsfonts,amssymb,stmaryrd}
\usepackage{galois}
\usepackage{mathtools}
% \usepackage{tikz}\usetikzlibrary{snakes,calc,matrix,arrows}
%\usepackage{tikzutil}
\usepackage[final]{listings}
\usepackage{theorems}

\parindent 0pt
\date{\today, \currenttime}

\newcommand*{\intersep}{\\}
\newcommand*{\interfill}{\\}
\newcommand*{\intrasep}{\\[2ex]}

\newcommand*{\prm}[1]{\fbox{#1}}

\newcommand*{\txmacroZ}[1]{\texttt{\string#1} $\rightarrow$ \fbox{#1} \intrasep}
\newcommand*{\txmacroOnOp}[1]{%
\texttt{\string#1} $\rightarrow$ \fbox{#1}\interfill
\texttt{\string#1[\prm{a}]} $\rightarrow$ \fbox{#1[\prm{a}]}\intrasep
}
\newcommand*{\txmacroOn}[1]{%
\texttt{\string#1\{\}} $\rightarrow$ \fbox{#1{}}\interfill
\texttt{\string#1\{\prm{a}\}} $\rightarrow$ \fbox{#1{\prm{a}}}\intrasep
}
\newcommand*{\txmacroTw}[1]{
\texttt{\string#1\{\}\{\}} $\rightarrow$ \fbox{#1{}{}}\interfill
\texttt{\string#1\{\prm{a}\}\{\}} $\rightarrow$ \fbox{#1{\prm{a}}{}}\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}} $\rightarrow$ \fbox{#1{\prm{a}}{\prm{b}}}\intrasep
}

\newcommand*{\macroREDEFz}[1]{do not use, redefine only %
  \fbox{\texttt{\string#1} $\rightarrow$ $#1$}\intrasep}
\newcommand*{\macroREDEFon}[1]{do not use, redefine only %
  \fbox{\texttt{\string#1\{AaBb\}} $\rightarrow$ $#1{AaBb}$}\intrasep}
\newcommand*{\macroZ}[1]{\texttt{\string#1} $\rightarrow$ $#1$\intrasep}
\newcommand*{\macroOnOp}[1]{%
\texttt{\string#1} $\rightarrow$ $#1$\interfill
\texttt{\string#1[\prm{a}]} $\rightarrow$ $#1[\prm{a}]$\intrasep
}
\newcommand*{\macroOn}[1]{%
\texttt{\string#1\{\}} $\rightarrow$ $#1{}$\interfill
\texttt{\string#1\{\prm{a}\}} $\rightarrow$ $#1{\prm{a}}$\intrasep
}
\newcommand*{\macroTw}[1]{
\texttt{\string#1\{\}\{\}} $\rightarrow$ $#1{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\}} $\rightarrow$ $#1{\prm{a}}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}$\intrasep
}
\newcommand*{\macroTwOp}[1]{
\texttt{\string#1\{\}} $\rightarrow$ $#1{}$\interfill
\texttt{\string#1[\prm{a}]\{\}} $\rightarrow$ $#1[\prm{a}]{}$\intersep
\texttt{\string#1\{\prm{b}\}} $\rightarrow$ $#1{\prm{b}}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}$\intrasep
}
\newcommand*{\macroTh}[1]{
\texttt{\string#1\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}$\intrasep
}
\newcommand*{\macroThOp}[1]{
\texttt{\string#1\{\}\{\}} $\rightarrow$ $#1{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\}} $\rightarrow$ $#1{\prm{b}}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\prm{c}\}} $\rightarrow$ $#1{\prm{b}}{\prm{c}}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}$\intrasep
}
\newcommand*{\macroFo}[1]{
\texttt{\string#1\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}$\intrasep
}
\newcommand*{\macroFoOp}[1]{
\texttt{\string#1\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{}{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\}\{\}} $\rightarrow$ $#1{\prm{b}}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\prm{c}\}\{\}} $\rightarrow$ $#1{\prm{b}}{\prm{c}}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}} $\rightarrow$ $#1{\prm{b}}{\prm{c}}{\prm{d}}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{\prm{d}}$\intrasep
}
\newcommand*{\macroFi}[1]{
\texttt{\string#1\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{}{}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}$\intrasep
}
\newcommand*{\macroFiOp}[1]{
\texttt{\string#1\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\}\{\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{}{}{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{b}}{}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{}{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\prm{c}\}\{\}\{\}} $\rightarrow$ $#1{\prm{b}}{\prm{c}}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{}{}$\intersep
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{\prm{d}}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}$\intrasep
}
\newcommand*{\macroSiOp}[1]{
\texttt{\string#1\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{}{}{}{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{b}}{}{}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{}{}{}{}$\intersep
\texttt{\string#1\{\prm{b}\}\{\prm{c}\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{b}}{\prm{c}}{}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{}{}{}$\intersep
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\}\{\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{\prm{d}}{}{}$\interfill
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{}$\intrasep
\texttt{\string#1[\prm{a}]\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{\prm{f}\}} $\rightarrow$ $#1[\prm{a}]{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{\prm{f}}$\intrasep
}
\newcommand*{\macroSi}[1]{
\texttt{\string#1\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{}{}{}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{}$\intrasep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{\prm{f}\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{\prm{f}}$\intrasep
}
\newcommand*{\macroSe}[1]{
\texttt{\string#1\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{}{}{}{}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\}\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{}{}{}{}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{}{}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{}{}{}{}$\intersep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{}{}{}$\interfill
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{}{}$\intrasep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{\prm{f}\}\{\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{\prm{f}}{}$\intrasep
\texttt{\string#1\{\prm{a}\}\{\prm{b}\}\{\prm{c}\}\{\prm{d}\}\{\prm{e}\}\{\prm{f}\}\{\prm{g}\}} $\rightarrow$ $#1{\prm{a}}{\prm{b}}{\prm{c}}{\prm{d}}{\prm{e}}{\prm{f}}{\prm{g}}$\intrasep
}


==> wgmacros-DOMS.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for DOMS   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\KPOS}[1][k]{\parensmathoper{Kpos}{#1}}

% now load general staff

\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%
%                %
%   temp stuff   %
%                %
%%%%%%%%%%%%%%%%%%

% \newcommand*{\pat}{\parensmathoper{pat}}
% \newcommand*{\ruleNode}{\parensmathoper{rule}}
% \newcommand*{\branchNode}{\parensmathoper{branch}}
% \newcommand*{\orNode}{\parensmathoper{or}}
% 
% %% TERM GRAPHS MACROS
% \newcommand*{\Roots}[1]{\mathcal{R}\mathclose{oot}_{#1}} %% root node
% \newcommand*{\Nds}[1]{\mathcal{N}_{#1}} %% graph nodes
% \newcommand*{\Lbl}[1][]{\parensmathoper{\mathcal{L}_{#1}}} %% label map
% \newcommand*{\Suc}[1][]{\parensmathoper{\mathcal{S}_{#1}}} %% successor map
% \newcommand*{\reach}[1]{\rightarrowtriangle_{#1}} %% reachability relation over positions of a term
% \newcommand*{\nreach}[1]{\not\rightarrowtriangle_{#1}} %% reachability relation over positions of a term
% 
% \newcommand*{\cv}[1]{\parensmathoper{cv}{#1}}


==> wgmacros-FLP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for FLPs   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\@ifpackageloaded{MnSymbol}{}{\PackageWarning{WGmacros}%
{Please load `MnSymbol' package explicitely in preamble}
\RequirePackage{MnSymbol}}
\makeatother
% \RequirePackage{listings}

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Small Step (Narrowing) Trees


\newcommand*{\NTdom}{\C}
\newcommand*{\NTedge}[3][]{\xRightarrow[{\extraArg{#3}{#1}}]{#2}}
\newcommand*{\NTspec}[3]{#1[#2/#3]} %% NT tree replacement
\newcommand*{\NTeq}{\cong_{\NTdom}} %% variance on tree
\newcommand*{\NTgeq}{\sqsupseteq} %% \NTleq^{-1}
\newcommand*{\NTglb}{\glbC}  %% g.l.b. on set of narrowing trees
\newcommand*{\NTleq}{\leqC} %% pre-order on narrowing trees
\newcommand*{\NTlub}{\lubC}  %% l.u.b. on set of narrowing trees
\newcommand*{\NTnleq}{\nleqC} %% pre-order on narrowing trees


\newcommand*{\botvar}[1][]{{\varrho_{#1}}}

\newcommand*{\botVsyms}{\Vsyms_{\botvar}}
\backcompatibility{\botVsym}{\botVsyms}
\newcommand*{\botTerms}[1][]{\SigTerms{\Csyms}{\Vsyms \cup \botVsyms}\ifempty{#1}{}{\Fbox{#1}}}
% \newcommand*{\botTerms}{\SigTerms{\Csyms}{\Vsyms \cup \botVsyms}}
\newcommand*{\botSubsts}{\botvar\Substs}

%% Incremental Answer Trees
\newcommand*{\IAT}{\mathbb{IRT}}
\newcommand*{\ipa}[5]{{}^{#1}/_{#2} \, #3 \ifempty{#4}{}{\, #4} \ifempty{#5}{}{\, #5}}
\newcommand*{\IATleq}{\Fbox{change}\preccurlyeq} %% pre-order on answer evolution trees
\newcommand*{\IATlub}[2]{{\ifempty{#2}{\bigcurlyvee #1}{#1 \curlyvee #2}}} %% l.u.b. on set of answer evolution trees 

%% Evolving Answer Trees
% private
\newcommand*{\EATabsSym}{\nu}
% public
\newcommand*{\EATF}{\F[\EATabsSym]}
\newcommand*{\EATTp}{\Tp[\EATabsSym]}
\newcommand*{\EATpreabs}[2][\emptysubst]{\parensmathoper{\EATabsSym^{#1}_{#2}}}%\mars
\newcommand*{\EATabs}[1][V]{\parensmathoper{\EATabsSym_{#1}}}%\mars
\newcommand*{\EATconc}[1][\pi]{\parensmathoper{\EATabsSym_{#1}^{\gamma}}}
\newcommand*{\EATedge}[1][\botvar]{\xrightarrow{#1}}
\newcommand*{\EATeq}{\mathrel{=_{\EAT}}} %% variance on answer evolution trees
\newcommand*{\EATevalrules}[4][V]{\syntaxoper{\xi^{\EATabsSym}_{#1}}{#3}{#2}^{#4}}
\newcommand*{\EATeval}[3]{\syntaxoperEXT{#2}{\evalSym^{\EATabsSym}}{\termres{#2}{#1}}{#3}}
\newcommand*{\EATgeq}{\succeq} %% \leqAET^{-1}
\monobioperator{\EATglb}{\curlywedge}{\bigcurlywedge} %% g.l.b. on set of answer evolution trees 
\newcommand*{\EATinterps}{\interpA[{\EAT[]}]}
\newcommand*{\EATinterp}{\I[\EATabsSym]}
\newcommand*{\EATleq}{\preccurlyeq} %% pre-order on answer evolution trees
\monobioperator{\EATlub}{\curlyvee}{\bigcurlyvee} %% l.u.b. on set of answer evolution trees 
\newcommand*{\EATnleq}{\npreccurlyeq} %% pre-order on answer evolution trees
\newcommand*{\EATnode}[3]{#1 \cdot \ifempty{#2}{}{#2 \cdot} #3}
\newcommand*{\EATspec}[4][V]{#2 [#3/#4]_{#1}}
\newcommand*{\EAT}[1][\zseq{x}]{{\mathbb{ERT}_{#1}}}
% \newcommand*{\EATgenericforest}{\mathcal{F}}
\newcommand*{\eleq}[1][\Fbox{V}]{\twoheadrightarrow_{#1}}% \precapprox}
\newcommand*{\shell}{\parensmathoper{\tau}} %% the shell of a term

%% Definitional Trees
\newcommand*{\pat}{\parensmathoper{pat}}
\newcommand*{\ruleNode}{\parensmathoper{rule}}
\newcommand*{\branchNode}{\parensmathoper{branch}}
\newcommand*{\orNode}{\parensmathoper{or}}

\newcommand*{\CurryEval}[6][]{\syntaxoper{Eval}{\extraArgSc{#2}{#1}}{} \xRightarrow[{#5}]{\extraArg{#3}{#4}} #6}

\newcommand*{\stricteq}{\mathbin{\mlst{=:=}}}
\newcommand*{\paralland}{\mathbin{\mlst{&}}}
\newcommand*{\seqand}{\mathbin{\mlst{&>}}}
\newcommand*{\success}{\mlst{success}}

%% TERM GRAPHS MACROS
\newcommand*{\Roots}[1]{\mathcal{R}\mathclose{oot}_{#1}} %% root node
\newcommand*{\Nds}[1]{\mathcal{N}_{#1}} %% graph nodes
\newcommand*{\Lbl}[1][\Fbox{g}]{\parensmathoper{\mathcal{L}_{#1}}} %% label map
\newcommand*{\Suc}[1][\Fbox{g}]{\parensmathoper{\mathcal{S}_{#1}}} %% successor map
\newcommand*{\reach}[1]{\rightarrowtriangle_{#1}} %% reachability relation over positions of a term
\newcommand*{\nreach}[1]{\nrightarrowtriangle_{#1}} %% reachability relation over positions of a term

%% Staff relative to (CRWL) term bottom

\newcommand*{\BotSym}{\bot}

\newcommand*{\BotCsyms}{\Csyms_{\BotSym}} %% constructor symbols
\newcommand*{\BotSyms}{\Fsyms_{\BotSym}} %%  symbols \cup black box

% \newcommand*{\cApprox}[1]{\tau_{\Cbox}(#1)}
\newcommand*{\cansw}[2]{{#1 \cdot #2}}%\talloblong\mathrel{}


\newcommand*{\strictvareq}{\mathrel{\doteq}}

% COMPATIBILITY

\backcompatibility{\BoxCsym}{\BotCsyms}
\backcompatibility{\BoxSym}{\BotSyms}
\backcompatibility{\Cbox}{\BotSyms}
\backcompatibility{\botSubst}{\botSubsts}
\newcommand*{\pansw}[2]{\Fbox{$#1 \cdot #2$}}%\talloblong\mathrel{}

% now load general staff

\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand*{\proglang}{\textsf{Curry}}
\renewcommand*{\paradigm}[1][]{#1\textsf{FLP}}


==> wgmacros-FP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for FLPs   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\IAT}{\mathbb{IAT}}
\newcommand*{\EAT}{\mathbb{EAT}}


\newcommand*{\cansw}[2]{#1 \cdot #2}%\talloblong\mathrel{}

% now load general staff

\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> wgmacros-TCCP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for TCCP   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\@ifpackageloaded{MnSymbol}{}{\PackageWarning{WGmacros}%
{Please load `MnSymbol' package explicitely in preamble}
\RequirePackage{MnSymbol}}
\makeatother

\input{wgmacros-support}


% now load general staff

\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand*{\MGCsym}{\mathbb{PC}} %% most general call set

\renewcommand*{\zseq}[2][n]{\vec{#2}}

\renewcommand*{\genrule}[2]{#1 \clauseif #2}

\renewcommand*{\paradigm}[1][]{the #1\ccp\ paradigm}
\renewcommand*{\proglang}{\tccp}
\renewcommand*{\program}{set of declarations}
\renewcommand*{\programs}{sets of declarations}
\renewcommand*{\progequiv}{declarations equivalence}%\progrule\
\renewcommand*{\progrule}{process declaration}%
% \renewcommand*{\progrules}{process declarations}
\renewcommand*{\query}[1][A]{\ifempty{#1}{P}{p}rogram}
\renewcommand*{\queries}[1][A]{\query[#1]s}
\renewcommand*{\deffun}[1][A]{process}
\renewcommand*{\deffuns}[1][A]{processes}
\renewcommand*{\expression}[1][A]{\ifempty{#1}{A}{a}gent}
\renewcommand*{\expressions}[1][A]{\ifempty{#1}{A}{a}gents}

\renewcommand*{\C}[1][]{\mathbb{M}_{#1}}
\renewcommand*{\topC}{\mathbf{M}}
\renewcommand*{\botC}{\{\ecrs\}}

% \renewcommand*{\eval}[4][\alpha]{\syntaxoper{\mathcal{A}^{#1}}{#3}{{#4}}} %% semantic evaluation
\renewcommand*{\Q}[2]{\ifempty{#2}{#1}{#2 \mathbin{.} #1}} % D.A -> \Q{A}{D}
\renewcommand*{\TpSym}{\mathC{D}}
\renewcommand*{\TrSym}{\mathC{P}} %% semantics tree in P
\renewcommand*{\evalSym}{\mathC{A}}

% In Tccp the function symbol signature does not exist, the predicates are
% the defined symbols and the constraint system signature provides the
% constructor symbols
\renewcommand*{\Fsyms}{\CSys,\Psyms}
\renewcommand*{\Csyms}{\Fbox{fix}\CSys} %% constructor symbols
\renewcommand*{\Dsyms}{\Psyms} %% defined symbols

\renewcommand*{\ProgSym}{D} %% generic program=set of decls
% Insieme degli insiemi di dichiarazioni: si usa \Progs
\renewcommand*{\ProgsSym}{\mathbb{D}} %\mathit{Progs}
\renewcommand*{\Progs}[1][\CSys]{\ProgsSym^{\Psyms}_{#1}} % \mathit{Progs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand*{\N}{\mathbb{N}}
\newcommand*{\R}{\mathbb{R}}
\newcommand*{\Z}{\mathbb{Z}}

\newcommand*{\D}{\prog} %% generic program Alias

\newcommand*{\CCSname}{Cylindric Constraint System}
\newcommand*{\CCSshortname}{Constraint System}
\newdefinition{CCSdef}[theorem]{\CCSname}
\newsmartprefix{CCS}{\CCSshortname}
\newsmartsprefix{CCS}{\CCSshortname s}

\newcommand*{\CylConSyst}[7]{\langle #1, \mathord{#2}, #3, #4, #5, \mathord{#6}, #7 \rangle}
\newcommand*{\CCS}{\CylConSyst{\CSdom}{\CSord}{\CSmerge}{\CStrue}{\CSfalse}{\Var}{\CShid{}{}}}

% Insieme degli agenti
\newcommand*{\Agents}[1][\CSys]{\mathbb{A}^{\Psyms}_{#1}}%\mathit{Agents}
% Insieme dei "programmi" NON SERVE

\newcommand*{\Conds}[1][\CSys]{\Lambda_{#1}}%\mathit{Agents}
\newcommand*{\ValConds}[1][\CSys]{\Delta_{#1}}%\mathit{Agents}


\newcommand*{\evalC}[3][\alpha]{\syntaxoper{\bar{\evalSym}^{#1}}{#2}{{#3}}} %compact eval
\newcommand*{\TpC}[3][\alpha]{\syntaxoper{\bar{\TpSym}^{#1}}{#2}{{#3}}}%compact Tp
\newcommand*{\FC}[2][\alpha]{\syntaxoper{\bar{\FSym}^{#1}}{#2}{}}%compact fixpoint

\newcommand*{\Conf}{\mathit{Conf}}% insieme di configurazioni
%\newcommand*{\PA}{\fbox{change to $\MGC$}}
\newcommand*{\clauseif}{\ensuremath{\mathrel{\mathord{:}\mathord{-}}}}
\newcommand*{\ra}{\rightarrow}
\newcommand*{\nra}{\not\rightarrow}
\newcommand*{\tccp}{\textit{tccp}}
\newcommand*{\ntcc}{\textit{ntcc}}
\newcommand*{\ccp}{\textit{ccp}}
\newcommand*{\cc}{\textit{cc}}
\newcommand*{\tcc}{\textit{tcc}}
\newcommand*{\hcc}{\textit{hcc}}
\newcommand*{\utcc}{\textit{utcc}}

%%OPERATORI TCCP%%

\newcommand*{\askip}{\mathord{\mathsf{skip}}}%agente skip
\newcommand*{\atell}{\parensmathoper{\mathsf{tell}}}%agente tell
%\newcommand*{\aask}{\parensmathoper{\mathsf{ask}}}%agente ask
\newcommand*{\aask}[1]{\mathop{\mathsf{ask}}\ifempty{#1}{}{(#1)\ra}}
\newcommand*{\asumask}[4][i]{\sum_{#1=1}^{#2}\aask{#3_{#1}}{#4}_{#1}}
\newcommand*{\anow}[3]{\tagnow\ifempty{#1}{} {\: #1 \tagthen #2\ifempty{#3}{}{\tagelse #3}}}
\newcommand*{\anowpar}[3]{\anow{(#1)}{#2}{#3}}
\newcommand*{\ahiding}[3][]{\mathop{\exists^{#1}{#2}} {#3}}
\newcommand*{\aparallel}[2]{#1 \parallel #2}
\newcommand*{\apcall}[2]{\mathit{#1}\ifempty{#2}{}{(\mathit{#2})}}

\newcommand*{\tagelse}{\mathrel{\mathsf{else}}}
\newcommand*{\tagnow}{\mathop{\mathsf{now}}}
\newcommand*{\tagthen}{\mathrel{\mathsf{then}}}


% \newcommand*{\ordtree}{\unlhd}
% \newcommand*{\emptytree}{\Box}

%%SEQUENZE REATTIVE%%

%\newcommand*{\R}{\mathit{R}}
%\newcommand*{\Sr}{\mathcal{S}}%dominio sequenze reattive classiche
%\newcommand*{\Rconn}{\mathbb{R}_{conn}} %insieme di sequenze reattive condizionali connesse

%%MASSIMALI

\backcompatibility{\M}{\C}
\backcompatibility{\Rm}{\C}%dominio sequenze reattive condizionali massimali
\backcompatibility{\leqM}{\leqC}
\backcompatibility{\lubM}{\lubC}%[2]{{\ifempty{#2}{\bigsqcup #1}{#1 \sqcup #2}}}
\backcompatibility{\glbM}{\glbC}%[2]{{\ifempty{#2}{\bigsqcap #1}{#1 \sqcup #2}}}
\backcompatibility{\botM}{\botC}
\backcompatibility{\topM}{\topC}
\backcompatibility{\latticeM}{\latticeC}
\backcompatibility{\cpoM}{\cpoC}

\newcommand*{\prefix}{\parensmathoper{prefix}}%op prefissi

\newcommand*{\parallelstore}[2]{\mathbin{\ifempty{#1}{\breve{\parallel}}{#1\mathrel{\breve{\parallel}} #2}}}
%parallel sequenze condizionali

%TUPLE CONDIZIONALI

\newcommand*{\seqHid}[2]{\mathop{\bar{\exists}}\nolimits_{#1} #2}
\newcommand*{\cs}[2]{ #1 \rightarrowtail #2}%\Yright\llparenthesis\rrparenthesis
\newcommand*{\csC}[3]{\cs{\cond{#1}{#2}}{#3}}
\newcommand*{\ecrs}{\epsilon} %seq. reattiva condizionale vuota

%da togliere:
% \newcommand*{\crs}[3]{\ifempty{#1}{}{#1 \Rightarrow} \pair{#2}{#3}} %tupla condizionale
% \newcommand*{\crsC}[4]{\crs{\cond{#1}{#2}}{#3}{#4}} % con condizioni esplicite
% \newcommand*{\rs}{\crs{}}
% \newcommand*{\ucoRrm}{\uco{\Rrm}{\ordRrm}}%uco sequenze massimali
% \newcommand*{\ucoRr}{\uco{\Rr}{\subseteq}}%uco sequenze
% \newcommand*{\ucoTree}{\uco{\Tree}{\ordTree}}%uco alberi


%%OPERATORI SU SEQUENZE REATTIVE%%

% \newcommand*{\seq}{\mathoper{Seq}}%costruisce la sequenza
%\newcommand*{\Conn}{\mathit{Conn}}%sequenze connesse
\newcommand*{\ed}{\boxtimes}
\newcommand*{\first}{\parensmathoper{first}}%primo store di una sequenza
\newcommand*{\last}{\parensmathoper{last}}%ultimo store di una sequenza
%\newcommand*{\inc}{\Omega} %insieme seq. inconsistenti
\newcommand*{\parallelseq}[2]{\mathbin{\ifempty{#1}{\bar{\parallel}}{#1\mathrel{\bar{\parallel}} #2}}}
%parallel sequenze condizionali
%\newcommand*{\addstore}[2]{\ifempty{#1}{\mathbin{\varoast}}{#1\mathbin{\varoast}#2}}%prop constraints operatore tran
%\newcommand*{\prop}[2]{\ifempty{#1}{\mathbin{\odot}}{#1\mathbin{\odot}}#2}%prop constraints
\newcommand*{\prop}[2]{#2\mathord{\downarrow_{#1}}}%prop constraints
%\newcommand*{\remcond}{\mathoper{RemoveConditions}}%rimuovere cond.
\newcommand*{\conscond}[2] {#1 \gg \ifempty{#1}{}{#2}}%consistenza di una condizione rispetto a uno store
\newcommand*{\nconscond}[2]{#1 \ngg \ifempty{#1}{}{#2}}%INconsistenza di una condizione rispetto a uno store
\newcommand*{\soddcond}[2] {#1 \rightModels\allowbreak \ifempty{#1}{}{#2}}%soddisfazione di una condizione rispetto a uno store
\newcommand*{\nsoddcond}[2]{#1 \nrightModels \ifempty{#1}{}{#2}}%INsoddisfazione di una condizione rispetto a uno store
\newcommand*{\stutt}[1]{\parensmathoper{\mathit{stutt}}{#1}}
%\newcommand*{\tran}[1]{\Downarrow_{#1}}  %operatore trasformazione
\newcommand*{\tran}[2]{#2\mathord{\Downarrow_{#1}}}
% \ifempty{#1}{\ifempty{#2}{\Downarrow}{\Downarrow_{#1}}}{#2\Downarrow_{#1}}}
%\newcommand*{\tranaux}[1]{\downarrow_{#1}}   %operatore trasformazione ausiliario
%\newcommand*{\uncond}{\mathbin{\otimes_{c}}}
\newcommand*{\uncond}{\mathbin{\otimes}}

%%CONSTRAINT SYSTEM%%

\newcommand*{\CSc}[1][c]{#1}
\newcommand*{\CSdom}{\mathcal{C}} %insieme di constraint
\newcommand*{\CSfalse}{\mathit{false}} %insieme di constraint
\newcommand*{\CShid}[2]{\mathop{\exists}\nolimits_{#1} #2}%exists
\newcommand*{\CSimp}{\mathrel{\vdash}}%implicazione
\newcommand*{\CSnimp}{\mathrel{\nvdash}}%implicazione
\newcommand*{\CSjoin}{\mathbin{\oplus}}%merge constraints
\newcommand*{\CSmerge}{\mathbin{\otimes}}%merge constraints
\newcommand*{\CSord}{\preceq}%contrario implicazione
\newcommand*{\CStrue}{\mathit{true}} %insieme di constraint
\newcommand*{\CSys}{\mathbf{C}} %constraint system
\newcommand*{\Var}{\mathit{Var}}%variabili

%%ABSTRACT CONSTRAINT SYSTEMS%%

\newcommand*{\ACSc}[1][c]{\hat{\CSc[{#1}]}}
\newcommand*{\ACSdom}{\hat{\CSdom}} %insieme di constraint
\newcommand*{\ACShid}[2]{\mathop{\hat\exists}\nolimits_{#1} #2}
\newcommand*{\ACSimp}{\mathrel{\hat\CSimp}}%implicazione
\newcommand*{\ACSnimp}{\mathrel{\hat\CSnimp}}%implicazione
\newcommand*{\ACSjoin}{\mathbin{\hat\CSjoin}}%merge constraints
\newcommand*{\ACSmerge}{\mathbin{\tilde\CSmerge}}%merge constraints
\newcommand*{\ACSord}{\mathrel{\hat{\CSord}}}
\newcommand*{\ACSys}{\hat{\CSys}} %constraint system
\newcommand*{\ACSfalse}{\hat{\CSfalse}}
\newcommand*{\ACStrue}{\hat{\CStrue}}

\newcommand*{\ACCS}{\CylConSyst{\ACSdom}{\ACSord}{\ACSmerge}{\ACStrue}{\ACSfalse}{\Var}{\ACShid{}{}}}

\newcommand*{\ACSimppn}{\mathrel{\tilde\vdash}}%implicazione positiva e negativa
\newcommand*{\ACSnimppn}{\mathrel{\tilde\nvdash}}%implicazione positiva e negativa

\newcommand*{\AseqHid}[2]{\mathop{\tilde{\exists}}\nolimits_{#1} #2}

\newcommand*{\ACScDual}[1][a]{\check{\CSc[{#1}]}}
\newcommand*{\ACSdomDual}{\check{\CSdom}} %insieme di constraint
\newcommand*{\ACSfalseDual}{\check{\CSfalse}}
\newcommand*{\ACShidDual}[2]{\mathop{\check\exists}\nolimits_{#1} #2}
\newcommand*{\ACSimpDual}{\mathrel{\check\CSnimp}}%implicazione
\newcommand*{\ACSnimpDual}{\mathrel{\check\CSimp}}%implicazione
\newcommand*{\ACSjoinDual}{\mathbin{\check\CSjoin}}%merge constraints
\newcommand*{\ACSmergeDual}{\mathbin{\check\CSmerge}}%merge constraints
\newcommand*{\ACSordDual}{\mathrel{\check{\CSord}}}
\newcommand*{\ACStrueDual}{\check{\CStrue}}
\newcommand*{\ACSysDual}{\check{\CSys}} %constraint system

\newcommand*{\ACCSDual}{\CylConSyst{\ACSdomDual}{\ACSordDual}{\ACSmergeDual}{\ACStrueDual}{\ACSfalseDual}{\Var}{\ACShidDual{}{}}}

\newcommand*{\ACSetac}{\tilde{\eta}}
\newcommand*{\ACSetam}{\check{\eta}}
\newcommand*{\ACSetapm}{\cond{\ACSetap}{\ACSetam}}
\newcommand*{\ACSetap}{\hat{\eta}}
\newcommand*{\ACSinjDual}[2]{#1 \mathbin{\check{\times}} #2}
\newcommand*{\ACSinj}[2]{#1 \mathbin{\hat{\times}} #2}


%%ABSTRACT REACTIVE SEQUENCE%%

%abstract sequences
\newcommand*{\latticeAM}{\lattice{\AMdom}{\leqAM}{\lubAM{}{}}{\glbAM{}{}}{\topAM}{\botAM}}
\newcommand*{\cpoAM}{\cpo{\AMdom}{\leqAM}}
\newcommand*{\leqAM}{\leqC}
\newcommand*{\AMdom}{\C^{\pm}}
\monobioperator{\glbAM}{\sqcap}{\bigsqcap}
\monobioperator{\lubAM}{\sqcup}{\bigsqcup}
\newcommand*{\botAM}{\botC}
\newcommand*{\topAM}{\topC^{\pm}}

%compact abstract sequences
\newcommand*{\latticeKAM}{\lattice{\KAMdom}{\leqKAM}{\lubKAM{}{}}{\glbKAM{}{}}{\topKAM}{\botKAM}}
\newcommand*{\cpoKAM}{\cpo{\KAMdom}{\leqKAM}}
\newcommand*{\leqKAM}{\leq}
\newcommand*{\KAMdom}{\tilde{\C}^{\pm}}
\monobioperator{\glbKAM}{\wedge}{\bigwedge}
\monobioperator{\lubKAM}{\vee}{\bigvee}
\newcommand*{\botKAM}{\botC}
\newcommand*{\topKAM}{\tilde{\topC}^{\pm}}

\newcommand*{\Acs}[3][n]{[\cs{#2}{#3}]^{#1}}
\newcommand*{\AcsC}[4][n]{[\cs{\cond{#2}{#3}}{#4}]^{#1}}
\newcommand*{\Astutt}[2][n]{[\parensmathoper{\mathit{stutt}}{#2}]^{#1}}

\newcommand*{\cond}[2]{(#1 ,\allowbreak #2)} %\,

\newcommand*{\AConds}[1][\CSys]{\tilde{\Lambda}_{#1}}%\mathit{Agents}
\newcommand*{\AValConds}[1][\CSys]{\tilde{\Delta}_{#1}}%\mathit{Agents}

%\newcommand*{\Ainc}{\Omega_{\alpha}} %insieme seq. inconsistenti
%\newcommand*{\ARr}{\Rr^{\alpha}}%dominio astratto sequenze

\newcommand*{\Aprop}[2]{\ifempty{#1}{\tilde{\downarrow}}{#2 \tilde{\downarrow}_{#1}}}%prop astratta constraints
\newcommand*{\Aparallelseq}[2]{\mathbin{\ifempty{#1}{\tilde{\parallel}}{#1 \mathrel{\tilde{\parallel}} #2}}}
\newcommand*{\Asoddcond}[2]{\mathrel{\ifempty{#1}{\mathrel{\tilde\rightModels}}{#1 \mathrel{\tilde\rightModels} #2}}}
%soddisfazione di una condizione rispetto a uno store
\newcommand*{\Ansoddcond}[2]{\ifempty{#1}{\tilde{\nrightModels}}{#1 \mathrel{\tilde{\nrightModels}} #2}}
\newcommand*{\Aconscond}[2]{\ifempty{#1}{\tilde\gg}{#1 \mathrel{\tilde{\gg}} #2}}
\newcommand*{\Anconscond}[2]{\ifempty{#1}{\tilde{\ngg}}{#1 \mathrel{\tilde{\ngg}} #2}}
\newcommand*{\Auncond}{\mathbin{\tilde{\otimes}}}

\newcommand*{\cmpt}{\parensmathoper{\kappa}}
\newcommand*{\cmptrev}{\parensmathoper{\kappa^{-1}}}

% \newcommand*{\ARrm}{\mathbb{R}_{m}^{\alpha}}%dominio sequenze astratte massimali
% \newcommand*{\ATree}{\mathbb{T}^{\alpha}}%dominio alberi astratti

%%SEMANTICS%%

%% behavior
\newcommand*{\BehaQ}[4][\mathit{ss}]{\syntaxoperEXT{#3}{\BehaSym^{\mathit{#1}}}{\Q{#3}{#4}}{#2}}
\newcommand*{\BehaFinQ}[4][\mathit{ss}]{\syntaxoperEXT{#3}{\BehaSym^{\mathit{#1}}_{F}}{\Q{#3}{#4}}{#2}}

%% concrete semantics
\newcommand*{\Aa}{\eval[]{}} % [2]{#1}{#2}sem agente
\newcommand*{\Dd}{\Tp[]} %[2]{#1}{#2}sem dich.
\newcommand*{\Pp}[2]{\ifempty{#2}{\Tr[]{#1}{}}{\Tr[]{#2}{#1}}}
\newcommand*{\Qq}[2]{\Q{#2}{#1}}
% [2]{\syntaxoper{\mathcal{P}}{\ifempty{#2}{{#1}}{\Q{#2}{#1}}}{}}%semantica sequenze reattive condizionali

%\newcommand*{\B}{\mathcal{B}}%base di un proc.
\newcommand*{\Ii}{\interpC}%dominio interpretazione di un prog.

%da spostare in un altro file??

\newcommand*{\AAa}[2]{\eval[\pm]{}{#1}{#2}}%sem agente
\newcommand*{\ADd}[2]{\Tp[\pm]{#1}{#2}}%sem dich.

\newcommand*{\interpKAM}{\interpC^{\pm}}%dominio interpretazione di un prog.

\newcommand*{\AF}{\F[\pm]}
\newcommand*{\AI}{\I[\pm]}
\newcommand*{\AS}{\Sz[\pm]}

%%ABSTRACTIONS%%

\newcommand*{\alplus}{\parensmathoper{\tau^{+}}}%alpha constraint system piu
\newcommand*{\gaplus}{\parensmathoper{\gamma^{+}}}%gamma constraint system piu

\newcommand*{\alminus}{\parensmathoper{\tau^{-}}}%alpha constraint system meno
\newcommand*{\gaminus}{\parensmathoper{\gamma^{-}}}%gamma constraint system meno

\newcommand*{\alpm}{\parensmathoper{\alpha^{\pm}}}%alpha CS sequenze
\newcommand*{\gapm}{\parensmathoper{\gamma^{\pm}}}%gamma CS sequenze

\newcommand*{\Kalpm}{\parensmathoper{\tilde{\alpha}}}%alpha sequenze
\newcommand*{\Kgapm}{ \parensmathoper{\tilde{\gamma}}}%gamma sequenze

==> wgmacros-TRS.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   Staff only for TRSs   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\@ifpackageloaded{MnSymbol}{}{\PackageWarning{WGmacros}%
{Please load `MnSymbol' package explicitely in preamble}
\RequirePackage{MnSymbol}}
\makeatother

\input{wgmacros-support}

% now load general staff
\input{wgmacros-general}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   overrides of general defs   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand*{\C}[1][]{\mathbb{LNT}_{#1}}
\renewcommand*{\MGCsym}{\mathbb{MGT}}

\renewcommand*{\proglang}{the \textsf{TRS} formalism}
\renewcommand*{\paradigm}[1][]{the #1\textsf{TRS} paradigm}
\renewcommand*{\program}{TRS}
\renewcommand*{\programs}{TRSs}
\renewcommand*{\expression}{term}
\renewcommand*{\expressions}{terms}
\renewcommand*{\ProgsSym}{\mathbb{R}}
\renewcommand*{\ProgSym}{\mathcal{R}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   Subject Specific macros   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newsmartprefix{rules}{Rules}

\newcommand*{\cansw}[2]{{#1 \cdot #2}}%\talloblong\mathrel{}


% linearized narrowing
\newcommand*{\linNarrows}[3][]{\xRightarrow[{\scriptscriptstyle\extraArg{#3}{#1}}]{\scriptscriptstyle #2}}
\newcommand*{\linNarrowsTo}[3][]{\starred{\linNarrows[{#1}]{#2}{#3}}}
\newcommand*{\linNarrowStep}[4][\genrule{l}{r}]{\linNarrows[{#1}]{#2, #3}{#4}}


% big-step/small-step behavior and program equivalence
\newcommand*{\BSBeha}{\Beha[\mathit{bs}]} %% concrete behavior
\newcommand*{\BSProgEq}{\ProgEquiv[\mathit{bs}]} % big step program equivalence
\newcommand*{\SSBeha}{\Beha} %% super-concrete behavior
\newcommand*{\SSProgEq}{\ProgEquiv[\mathit{ss}]} % small step program equivalence

% relaxed narrowing tree
\newcommand*{\RNTdom}[1][]{\mathbb{LNT}_{#1}} %% relaxed narrowing trees
\newcommand*{\RNTpaths}{\Tpaths} %% path set for a relaxed narrowing tree
\newcommand*{\RNTlub}{\lubC}  %% l.u.b. on set of relaxed narrowing trees
\newcommand*{\RNTglb}{\glbC}  %% g.l.b. on set of relaxed narrowing trees
\newcommand*{\RNTleq}{\leqC}  %% ≤ on set of relaxed narrowing trees
\newcommand*{\WRNTdom}{\C} %% well-formed relaxed narrowing trees
\newcommand*{\RNTspec}[3]{#1[#2/#3]} %% RNT tree replacement
\newcommand*{\RNTspecRel}[4]{#1;#2;#3 \vdash #4} %% RNT specialization relation
\newcommand*{\vvars}[1]{\parensmathoper{\overrightarrow{var}}{#1}} %% term variables as a vector
\newcommand*{\dmgu}{\parensmathoper{\overleftarrow{mgu}}} % mgu stable on the firts argument
\newcommand*{\revSubst}[1]{#1^{-1}}

% relax narrowing sequence -> rewriting
\newcommand*{\RNseqToRew}[1]{\lfloor #1 \rfloor} % from relaxed narrowing sequences to rewriting derivations - cambiare nome macro


\newcommand*{\botvar}[1][]{{\varrho_{#1}}}

\newcommand*{\botVsyms}{\Vsyms_{\botvar}}




%%%%%%%%% da cancellare
\backcompatibility{\cR}{\prog} %% generic program Alias
\newcommand*{\narrowsRelax}[4]{\Fbox{USE \texttt{\string\linNarrows}}\xRightarrow[#1 \ifempty{#2}{}{, #2}]{#3 \ifempty{#4}{}{, #4}}} % rule, delinearizer, position, subst,
\newcommand*{\narrowsRelaxTo}[2]{\starred{\narrowsRelax{#1}{}{#2}{}}} % delinearizer, subst
\newcommand*{\narrowsRelaxStep}[4]{\Fbox{USE \texttt{\string\linNarrowStep}}\xRightarrow[#1 \ifempty{#2}{}{, #2}]{#3 \ifempty{#4}{}{, #4}}} % rule, delinearizer, position, subst,
% \backcompatibility{\NTpaths}{\Tpaths}
% \backcompatibility{\glbNT}{\glbC}
% \backcompatibility{\glbRND}{\glbC}
% \backcompatibility{\leqNT}{\leqC}
% \backcompatibility{\leqRND}{\leqC}
% \backcompatibility{\lubNT}{\lubC}
% \backcompatibility{\lubRND}{\lubC}
% \backcompatibility{\nleqRND}{\nleqC}
% \newcommand*{\Dstep}[3]{\Fbox{C}\langle #1, #2, #3 \rangle} %% RND step
% \newcommand*{\NTdom}{\Fbox{C}\mathbb{RNT}} %% relaxed narrowing trees
% \newcommand*{\RNDdom}{\Fbox{C}\mathbb{RND}} %% relaxed narrowing derivations
% \newcommand*{\WRNTdom}[1][]{\mathbb{RNT}_{#1}} %% well-formed relaxed narrowing trees
% \newcommand*{\prefixRND}[1]{\Fbox{C}\mathoper{prefix}(#1)} %% set of prefixes of a derivation


==> wgmacros-absint.tex <==
\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%   DOMAINS and orders   %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\lattice}[6]{{(#1, \, \mathord{#2}, \,
\annote{$\vee$}\mathord{#3}, \, \mathord{#4}, \,
\annote{$\top$}\mathord{#5}, \, \mathord{#6})}}

% Generic Concrete Domain (for preliminaries)

\newcommand*{\CC}{\mathbb{C}}
\newcommand*{\leqCC}{\sqsubseteq} %% order on Concrete Domain
\newcommand*{\nleqCC}{\nsqsubseteq} %% negated order on Concrete Domain
\monobioperator{\lubCC}{\sqcup}{\bigsqcup}
\monobioperator{\glbCC}{\sqcap}{\bigsqcap}
\newcommand*{\botCC}{\bot} %% bottom of Concrete Domain
\newcommand*{\topCC}{\top} %% top of Concrete Domain

\newcommand*{\cpoCC}{\cpo{\CC}{\leqCC}}
\newcommand*{\latticeCC}{\lattice{\CC}{\leqCC}{\lubCC{}{}}{\glbCC{}{}}{\topCC}{\botCC}}

% Default Concrete Domain (for paper body, to be localized)

\newcommand*{\lubCbigsym}{\bigsqcup}
\newcommand*{\glbCbigsym}{\bigsqcap}
\newcommand*{\lubCsym}{\sqcup}
\newcommand*{\glbCsym}{\sqcap}

\newcommand*{\C}{\CC}
\newcommand*{\leqC}{\leqCC}
\newcommand*{\geqC}{\sqsupseteq}
\newcommand*{\nleqC}{\nleqCC}
\monobioperator{\lubC}{\lubCsym}{\lubCbigsym}
\monobioperator{\glbC}{\glbCsym}{\glbCbigsym}
\newcommand*{\botC}{\botCC}
\newcommand*{\topC}{\topCC}

\newcommand*{\cpoC}{\cpo{\C}{\leqC}}
\newcommand*{\latticeC}{\lattice{\C}{\leqC}{\lubC{}{}}{\glbC{}{}}{\topC}{\botC}}

% Generic Abstract Domain (for preliminaries)

\renewcommand*{\AA}{\mathbb{A}}
\newcommand*{\leqAA}{\leq} %% order on Abstract Domain
\newcommand*{\nleqAA}{\nleq} %% order on Abstract Domain
\monobioperator{\lubAA}{\vee}{\bigvee}
\monobioperator{\glbAA}{\wedge}{\bigwedge}
\newcommand*{\botAA}{\bot} %% bottom of Abstract Domain
\newcommand*{\topAA}{\top} %% top of Abstract Domain

\newcommand*{\cpoAA}{\cpo{\AA}{\leqAA}}
\newcommand*{\latticeAA}{\lattice{\AA}{\leqAA}{\lubAA{}{}}{\glbAA{}{}}{\topAA}{\botAA}}

% Default Concrete Domain (for paper body, to be localized)

\newcommand*{\lubAbigsym}{\bigvee}
\newcommand*{\glbAbigsym}{\bigwedge}
\newcommand*{\lubAsym}{\vee}
\newcommand*{\glbAsym}{\wedge}

\newcommand*{\A}{\AA}
\newcommand*{\leqA}{\leqAA}
\newcommand*{\nleqA}{\nleqAA}
\monobioperator{\lubA}{\lubAsym}{\lubAbigsym}
\monobioperator{\glbA}{\glbAsym}{\glbAbigsym}
\newcommand*{\botA}{\botAA}
\newcommand*{\topA}{\topAA}

\newcommand*{\cpoA}{\cpo{\A}{\leqA}}
\newcommand*{\latticeA}{\lattice{\A}{\leqA}{\lubA{}{}}{\glbA{}{}}{\topA}{\botA}}

\newcommand*{\al}{\parensmathoper{\alpha}}
\newcommand*{\ga}{\parensmathoper{\gamma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               %
%   Names of Standard Domains   %
%                               %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\POS}{\ensuremath{\mathcal{POS}}}

\newcommand*{\POSpreabs}[1][]{\parensmathoper{\Gamma_{#1}}}
\newcommand*{\POSabs}{\parensmathoper{\alpha_{\Gamma}}}
\newcommand*{\POSconc}{\parensmathoper{\gamma_{\Gamma}}}
\newcommand*{\POSlub}{\lubA}
\newcommand*{\POSglb}{\glbA}
\newcommand*{\POSleq}{\leqA}
\newcommand*{\POSrestrict}[2]{{#1}|_{#2}}
\newcommand*{\POSTp}{\Tp[g]}
\newcommand*{\POSinterp}{\I[g]}
\newcommand*{\POSeval}{\eval[g]}

\newcommand*{\Iff}{\leftrightarrow}

% still to be organized

\newcommand*{\KCTerms}[1][\KVsyms]{\SigTerms{\Csyms}{\Vsyms\cup #1}} %[1][\Fsyms]{\TermsSym(#1, )} %% terms
\newcommand*{\KI}{{\I[\kappa]}}
\newcommand*{\KSz}{\Sz[\kappa]}
\newcommand*{\KTerms}[1][\KVsyms]{\Terms[{\Vsyms\cup #1}]} %[1][\Fsyms]{\TermsSym(#1, )} %% terms
\newcommand*{\KTp}{\Tp[\kappa]}
\newcommand*{\KVsyms}{\widehat{\Vsyms}}
\newcommand*{\Kcut}[2][k]{#2 \lightning_{#1}}
\newcommand*{\Keval}{\eval[\kappa]}
\newcommand*{\depthk}[1][k]{\ensuremath{\mathit{depth}(#1)}}


==> wgmacros-caterina.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> wgmacros-fboxed-defaults.tex <==

\renewcommand*{\C}{\Fbox{$\CC$}}
\renewcommand*{\leqC}{\Fbox{$\leqCC$}}
% \renewcommand*{\geqC}{\Fbox{$\geqCC$}}
\renewcommand*{\lubC}[2]{\Fbox{$\lubCC{#1}{#2}$}}
\renewcommand*{\glbC}[2]{\Fbox{$\glbCC{#1}{#2}$}}
\renewcommand*{\botC}{\Fbox{$\botCC$}}
\renewcommand*{\topC}{\Fbox{$\topCC$}}

\renewcommand*{\A}{\Fbox{$\AA$}}
\renewcommand*{\leqA}{\Fbox{$\leqAA$}}
\renewcommand*{\lubA}[2]{\Fbox{$\lubAA{#1}{#2}$}}
\renewcommand*{\glbA}[2]{\Fbox{$\glbAA{#1}{#2}$}}
\renewcommand*{\botA}{\Fbox{$\botAA$}}
\renewcommand*{\topA}{\Fbox{$\topAA$}}


==> wgmacros-general.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                         %
%   General definitions   %
%                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input{wgmacros-absint}
\input{wgmacros-math}
\input{wgmacros-misc}
\input{wgmacros-semantics}


==> wgmacros-giovanni.tex <==
%% Small-steps Tree
\backcompatibility{\rootT}{\Troot} %% node root
\backcompatibility{\stepsT}{\Tsteps} %% node steps
\backcompatibility{\Npaths}{\Tpaths} %% path set for a narrowing tree
\newcommand*{\Npansw}{\Fbox{giovanni}\parensmathoper{\mathcal{A}nsw}} %% small-step partial answers
\newcommand*{\Nrules}[3][]{\Fbox{giovanni}\evalrules[{#1}]{#3}{#2}}

\backcompatibility{\Nnode}{\Tnode} %% NT node
\newcommand*{\Nstep}[3]{\Fbox{giovanni}\triple{#1}{#2}{#3}} %% NT step
\newcommand*{\Ninterp}{\Fbox{change to I[]}\I[]} %% NT generic interpretation

\newcommand*{\step}[3]{\Fbox{giovanni}\xrightarrow[#2,#3]{#1}} %% DA TOGLIERE
\newcommand*{\compose}{\Fbox{giovanni}\otimes} % DA TOGLIERE
\newcommand*{\Teqn}{\Fbox{giovanni}\parensmathoper{Eqn}}  %% DA TOGLIERE

%% GRAPHICAL UTILITIES ---------------------------------------

\newcommand*{\branchlabels}[2]{
edge from parent 
  node[font=\scriptsize,above,sloped] {\Fbox{giovanni}#1} 
  node[font=\scriptsize,below,sloped] {#2}
} %% two-side labelled edge

\newcommand*{\branchepsilon}{\branchlabels{\Fbox{giovanni}$\emptysubst$}{$\emptysubst$}} %% two-side \epsilon labelled edge


%% MISC ----------------------------------------
\newcommand*{\focus}[1]{{\color{red!80!black}\Fbox{giovanni}#1}}
\backcompatibility{\vseq}{\zseq}
\newcommand*{\tuple}[1]{\Fbox{cambiare}\langle #1 \rangle}




==> wgmacros-laura.tex <==



==> wgmacros-luca.tex <==
%% DA DECIDERE e/o SISTEMARE %%%%%%%%%%%%%%%
\newcommand*{\Tspec}[3]{#1[#2/#3]}

\newcommand*{\TAbsStep}[4]{\Fbox{cambiare}\langle #1, #2, #3 \rangle} %% an abstract relaxed-step in a tree

\newcommand*{\csSubsts}[2]{\overline{\chi}(#1, #2)}

\newcommand*{\PAtrs}[3]{#1 \cdot #2 \cdot #3}

\newcommand*{\CS}{CS} %% Context Sensitive
\newcommand*{\cs}{\chi} %% Context Sensitive label
\newcommand*{\csTerm}[2][]{\chi\ifempty{#2}{}{(#2)_{#1}}} %% CS term abstraction
\newcommand*{\csTree}[1]{\chi\ifempty{#1}{}{(#1)}} %% CS tree abstraction
\newcommand*{\csInterp}[1]{\chi\ifempty{#1}{}{(#1)}} %% CS domain abstraction

\newcommand*{\nProgEquiv}[3][]{#2 \not\thickapprox_{#1} #3}
\newcommand*{\nSSProgEq}{\nProgEquiv[\mathit{ss}]} % small step program equivalence


% random TO BE ORDERED
\newcommand*{\evl}[3][\alpha]{\syntaxoper{\evalSym^{#1}}{#2}{#3}} %% semantic evaluation
\newcommand*{\rt}{\parensmathoper{rt}} %% node root
\newcommand*{\Tmgu}{\parensmathoper{\widetilde{mgu}}} % 
\newcommand*{\Trelax}[2]{\parensmathoper{relax}{#1,#2}} %% relaxed splitting of a tree-subst
\newcommand*{\Tsubs}{\parensmathoper{subs}} %% subst induced by all the roots in a tree-subst
\newcommand*{\linearize}{\parensmathoper{lin}} % term linearization 
\newcommand{\partialfunc}[3]{#1\colon #2 \rightharpoonup #3} % partial function
\newcommand*{\pos}[2][]{\mathcal{O}_{#1}(#2)} %% term positions set 
\newcommand*{\Nspec}[3]{#1[#2/#3]} %% NT tree replacement

\newcommand*{\lubRS}{\mathbin{\downarrow}} % oppure mathrel?


\newcommand*{\RNTbranchlabels}[2]{
edge from parent[double]
  node[font=\scriptsize,above,sloped] {#1} 
  node[font=\scriptsize,below,sloped] {#2}
} %% two-side labelled edge

\newcommand*{\RNTbranchepsilon}{\RNTbranchlabels{$\emptysubst$}{$\emptysubst$}} %% two-side \epsilon labelled edge

% % \newcommand*{\Sem}[2][]{\syntaxoper{\mathcal{S}^{#1}}{#2}{}} % a semantics S
% 


==> wgmacros-math.tex <==
\newcommand*{\dfn}{\coloneq}
\newcommand*{\revdfn}{\eqqcolon}

\makeatletter
\@ifpackagelater{mathtools}{2011/02/12}{%
\DeclarePairedDelimiterX{\set}[2]{\{}{\}}{#1\ifempty{#2}{}{\,\delimsize\vert\, #2}}
\DeclarePairedDelimiterX{\mset}[2]{\langle}{\rangle}{#1\ifempty{#2}{}{\,\delimsize\vert\, #2}}
}{%
\PackageWarning{WGmacros}{The version of `mathtools' package is too old, expect wrong output}
\DeclarePairedDelimiter{\set}{\{}{|}
\DeclarePairedDelimiter{\mset}{\langle}{|}
}
\makeatother


\newcommand*{\zseq}[2][n]{\overrightarrow{{#2}_{#1}}} %% indexed (short) sequence
\newcommand*{\seq}[2][n]{{#2}_{1}, \dots, {#2}_{#1}} %% indexed sequence
\newcommand*{\hoseq}[3][n]{#2{{#3}_{1}}, \dots, #2{{#3}_{#1}}}


\newcommand*{\PowerSet}[1]{\mathop{\powerset}(#1)}
\newcommand*{\FinPowerSet}[1]{\mathop{\powerset_{f}}(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                 %
%   Macros that some package may already provide  %
%                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\mathoper}[1]{\mathop{\mathit{#1}}\nolimits}

\providecommand*{\pair}[2]{{\langle #1, \, #2 \rangle}}
\providecommand*{\triple}[3]{{\langle #1, \, #2, \, #3 \rangle}}
\providecommand*{\quadruple}[4]{{\langle #1, \, #2, \, #3, \, #4 \rangle}}

\providecommand*{\true}{\mathit{true}}       %% simbolo di costante logica (T)
\providecommand*{\false}{\mathit{false}}     %% simbolo di costante logica (F)
\providecommand*{\id}[1][]{\mathit{id}_{#1}} %% funzione identica

\providecommand*{\True}{\mathit{True}}
\providecommand*{\False}{\mathit{False}}

\providecommand*{\nimplies}{\nRightarrow}
\renewcommand*{\implies}{\Rightarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                 %
%   Symbols that some package like MnSymbol may already provide   %
%                                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ProvideWarnCommand{\powerset}{\wp} 
\ProvideWarnCommand{\llbracket}{[\![}
\ProvideWarnCommand{\rrbracket}{]\!]}

\ProvideWarnCommand{\coloneqq}{\mathrel{\vcentcolon=}} %% :=
\ProvideWarnCommand{\coloneq}{\mathrel{\coloneqq}} 
\ProvideWarnCommand{\eqqcolon}{\mathrel{=\vcentcolon}} % =:

% Negated symbols
\ProvideWarnCommand{\ngg}{\not\gg} 
\ProvideWarnCommand{\nin}{\notin}
\ProvideWarnCommand{\notin}{\not\in}
\ProvideWarnCommand{\npreccurlyeq}{\not\preccurlyeq}
\ProvideWarnCommand{\nsimeq}{\not\simeq}
\ProvideWarnCommand{\nsqsubseteq}{\not\sqsubseteq}
\ProvideWarnCommand{\nrightarrowtriangle}{\not\rightarrowtriangle}
\ProvideWarnCommand{\nRightarrow}{\not\Rightarrow} 


==> wgmacros-misc.tex <==
\makeatletter
\@ifpackageloaded{listings}{
    \newcommand*{\mlst}[1]{\mbox{\lstinline[multicols=]`#1`}}
}{
    \newcommand*{\mlst}[1]{\fbox{\fbox{load package listings}\texttt{\string#1}}}
}
\makeatother

\providecommand*{\currenttime}{\fbox{NO TIME package}}
\providecommand*{\mathscr}{\PackageWarning{WGmacros}{no mathscr font}\mathcal} 
\providecommand*{\mathfrak}{\PackageWarning{WGmacros}{no mathfrak font}\mathcal} 

\providecommand*{\eg}   {e.g.} 
\providecommand*{\etc}  {\emph{etc}.}
\providecommand*{\ie}   {i.e.,} 
\providecommand*{\resp} {respectively}
\providecommand*{\st}   {s.t.}
\providecommand*{\wrt}  {w.r.t.}
\providecommand*{\wlg}  {w.l.o.g.}
% \providecommand*{\Wlog} {\wlg}
% 
\newcommand*{\paradigm}[1][] {\Fbox{default #1 paradigm}}
\newcommand*{\proglang}{\Fbox{default programming language}}
\newcommand*{\program}[1][A]{\ifempty{#1}{P}{p}rogram}
\newcommand*{\programs}[1][A]{\program[#1]s}
\newcommand*{\progequiv}{\program\ equivalence}
\newcommand*{\progequivs}{\progequiv s}
\newcommand*{\progrule}{\program\ rule}
\newcommand*{\progrules}{\progrule s}
\newcommand*{\query}[1][A]{\ifempty{#1}{Q}{q}uery}
\newcommand*{\queries}[1][A]{\ifempty{#1}{Q}{q}ueries}
\newcommand*{\expression}[1][A]{\ifempty{#1}{E}{e}xpression}
\newcommand*{\expressions}[1][A]{\expression[#1]s}
\newcommand*{\deffun}[1][A]{\ifempty{#1}{defined }{}function}
\newcommand*{\deffuns}[1][A]{\deffun[#1]s}


\providecommand*{\bibURLext}[2]{\draft{CONSIDER convert bib entry with `url' field!}Available at URL: \href{#1}{\texttt{#2}}}
\providecommand*{\bibURL}[1]{\draft{CONSIDER convert bib entry with `url' field!}Available at URL: \href{#1}{\texttt{#1}}}
\providecommand*{\href}[2]{\wgmWarn{\href}\underline{#2}}

\providecommand*{\email}[1]{\texttt{#1}}

\newcommand*{\xcite}[1]{[{#1}]}

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{color}

\newcommand*{\Fbox}{\fcolorbox{black}{yellow}}
\newcommand*{\Flbox}{\fcolorbox{black}{lightyellow}}
\newcommand*{\Dbox}[1]{\draft{\Fbox{#1}}}

\definecolor{aliciacolor}{RGB}{0,125,0}

\newcommand{\Ago}[2][]{\hole{\colorbox{yellow}{Santi} #1 \quad #2}}
\newcommand{\Marco}[2][]{{\color{blue}\hole{\colorbox{yellow}{Marco} #1 \quad #2}}}
\newcommand{\Maria}[2][]{\hole{\colorbox{yellow}{Maria} #1 \quad #2}}
\newcommand{\Moreno}[2][]{\hole{\colorbox{yellow}{Moreno} #1 \quad #2}}

\newcommand{\Alicia}[2][]{\hole{\textbf{#1}\hfill{\color{aliciacolor}\textbf{Alicia}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\Giovanni}[2][]{\hole{\textbf{#1}\hfill{\color{blue}\textbf{Giovanni}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}

% nonstandard color names

\RequirePackage{xcolor}

\newcommand{\FromTo}[2]{\csname#1\endcsname[\colorbox{pink}{@#2}]}

\newcommand{\Laura}[2][]{\hole{\textbf{#1}\hfill{\color{violet}\textbf{Laura}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\Luca}[2][]{\hole{\textbf{#1}\hfill{\color{orange}\textbf{Luca}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}
\newcommand{\MarcoA}[2][]{\hole{\textbf{#1}\hfill{\color{orange}\textbf{MarcoA}}\\[-1.7ex]\rule{\linewidth}{0.5mm}\\ #2}}

% \newcommand{\AtAlicia}{\FromTo{Marco}{Alicia}}%[1]\Marco[\colorbox{pink}{@Alicia}]{#1}}
% \newcommand{\AtGiovanni}{\FromTo{Marco}{Giovanni}}%[1]{\Marco[\colorbox{pink}{@Giovanni}]{#1}}
% \newcommand{\AtLaura}{\FromTo{Marco}{Laura}}%[1]{\Marco[\colorbox{pink}{@Laura}]{#1}}
% \newcommand{\AtLuca}{\FromTo{Marco}{Luca}}%[1]{\Marco[\colorbox{pink}{@Luca}]{#1}}



==> wgmacros-semantics.tex <==
\makeatletter
\providecommand{\ifempty}[3]{\def\@@@temp{#1}\ifx\@@@temp\@empty#2\else#3\fi}
\@ifpackageloaded{mathtools}{}{\PackageWarning{WGmacros}%
{Please load `mathtools' package explicitely in preamble}
\RequirePackage{mathtools}}
\makeatother

\input{wgmacros-support}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%   DOMAINS and orders   %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\cpo}[2]{{(#1, \, \mathord{#2})}}

\newcommand*{\interpC}[1][]{\mathbb{I}_{#1}} %% interpretations
\newcommand*{\interpA}[1][\A]{\mathbb{I}_{#1}} %% interpretations
\newcommand*{\leqIc}{\leqC} %% order on interpretetions
\newcommand*{\leqIa}{\leqA} %% order on interpretetions
\newcommand*{\nleqIc}{\nleqC} %% order on interpretetions
\newcommand*{\nleqIa}{\nleqA} %% order on interpretetions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       %
%   TERMS (signature, positions, ...)   %
%                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% private (just for redefinition)
\newcommand*{\mathT}{\mathcal}
\newcommand*{\TermsSym}{\mathT{T}}
\newcommand*{\LinTermsSym}{\mathT{L}\scriptstyle{\TermsSym}}
\newcommand*{\twoParsDenot}[3]{\mathop{#1}(#2, #3)}
% public

\newcommand*{\SigTerms}[2]{\twoParsDenot{\TermsSym}{#1}{#2}}
\newcommand*{\LinSigTerms}[2]{\twoParsDenot{\LinTermsSym}{#1}{#2}}

\newcommand*{\Psyms}{\Pi}       %% predicate symbols (signature)
\newcommand*{\Fsyms}{\Sigma}    %% function symbols (signature)
\newcommand*{\Csyms}{\mathT{C}} %% constructor symbols
\newcommand*{\Dsyms}{\mathT{D}} %% defined symbols
\newcommand*{\Vsyms}{\mathT{V}} %% variable symbols
\backcompatibility{\Fsym}{\Fsyms}
\backcompatibility{\Csym}{\Csyms}
\backcompatibility{\Dsym}{\Dsyms}
\backcompatibility{\Vsym}{\Vsyms}




%% terms
\newcommand*{\Terms}[1][\Vsyms]{\SigTerms{\Fsyms}{#1}}
%% constructor terms
\newcommand*{\CTerms}[1][\Vsyms]{\SigTerms{\Csyms}{#1}}

%% Linear terms
\newcommand*{\LinTerms}[1][\Vsyms]{\LinSigTerms{\Fsyms}{#1}}
%% Linear constructor terms
\newcommand*{\LinCTerms}[1][\Vsyms]{\LinSigTerms{\Csyms}{#1}} 

\newcommand*{\leqT}{\preceq} %% order on terms

% \newcommand*{\leqP}{\fbox{change}\preceq} %% order on positions
% \newcommand*{\pos}[2][]{\mathcal{O}_{#1}(#2)} %% term positions set 
\newcommand*{\append}{\cdot} %% append
\newcommand*{\replace}[3]{#1[#2]_{#3}} %% term replacement
\newcommand*{\rootPos}{\Lambda} %% root position
\newcommand*{\subterm}[2]{#1|_{#2}} %% subterm

\newcommand*{\vars}[1]{\parensmathoper{var}{#1}} %% term variables
\newcommand*{\fresh}{\ll} %% fresh variant

\newcommand*{\termres}[2]{{#1} \ifempty{#2}{}{\triangleright {#2}}}

\newcommand*{\call}[3]{\termres{\mathit{#1}\ifempty{#2}{}{(\mathit{#2})}}{#3}}
\newcommand*{\mgc}[4][n]{\call{#2}{\mbox{$\zseq[#1]{#3}$}}{#4}}

%% program (rewrite) rule
\newcommand*{\genrule}[2]{#1 \rightarrow #2}
\newcommand*{\prule}[3]{\genrule{\mathit{#1}\ifempty{#2}{}{(\mathit{#2})}}{#3}}

\newcommand*{\mghead}[3][n]{\mathit{#2}\ifempty{#3}{}{(\zseq[#1]{\mathit{#3}})}}
\newcommand*{\mgrule}[4][n]{\genrule{\mghead[#1]{#2}{#3}}{#4}}

% \newcommand*{\letop}[2]{\mathop{\mathit{let}} #1 \mathrel{\mathit{in}} #2 } %% let constr. (abstract syntax)

%%%%%%%%%%%%%%%%%%%%%
%                   %
%   SUBSTITUTIONS   %
%                   %
%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\Substs}{\mathit{Substs}}
\newcommand*{\CSubsts}{\Csyms\Substs} %% constructor substitutions
\newcommand*{\MGCsym}{\mathbb{MGC}}
\newcommand*{\MGC}[1][]{\MGCsym_{#1}} %% most general call set

\newcommand*{\leqS}{\preceq} %% order on substitutions
\newcommand*{\gtS}{\succ}    %% order on substitutions
\newcommand*{\eqS}{\simeq}    %% order on substitutions
\newcommand*{\neqS}{\nsimeq}    %% order on substitutions
\newcommand*{\lubS}{\mathbin{\uparrow}} % oppure mathrel?

\newcommand*{\emptysubst}{\varepsilon} %% empty substitution
\newcommand*{\dom}{\parensmathoper{dom}} %% domain
\newcommand*{\range}{\parensmathoper{range}} %% range
\newcommand*{\img}{\parensmathoper{img}}
\backcompatibility{\domrestriction}{\restrict}
\newcommand*{\restrict}[2]{{#1}\mathord{\restriction}_{#2}} %% domain restriction
\newcommand*{\restrictVars}[2]{\restrict{#1}{\vars{#2}}}

%%%%%%%%%%%%%%%%
%              %
%   PROGRAMS   %
%              %
%%%%%%%%%%%%%%%%

\newcommand*{\ProgsSym}{\mathbb{P}}
\newcommand*{\Progs}[1][\Fsyms]{\ProgsSym_{#1}} % \mathit{Progs}

\newcommand*{\ProgSym}{P}
\newcommand*{\prog}[1][]{\ensuremath{\ProgSym_{\mathit{#1}}^{}}} %% generic program
\renewcommand*{\P}{\prog} %% generic program Alias

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             %
%   REWRITING AND NARROWING   %
%                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \RequirePackage{theorems}
\providecommand*{\starred}[2][*] {\wgmWarn{\starred}\mathrel{\mathord{#2}{}^{#1}}}


\newcommand*{\rewriteStep}[2][\genrule{l}{r}]{\xrightarrow[{#1}]{#2}}
% \newcommand*{\rewriteStep}[2][\genrule{l}{r}]{\xrightarrow[{\scriptscriptstyle #1}]{\scriptscriptstyle #2}}
\newcommand*{\rewrites}[1][]{\rewriteStep[{#1}]{}}
\newcommand*{\rewritesTo}[1][]{\starred{\rewrites[{#1}]}}
\newcommand*{\nrewrites}{\nrightarrow}


\newcommand*{\narrows}[2][]{\mathrel{\mathop{\leadsto}\limits^{\scriptscriptstyle #2}_{\scriptscriptstyle #1}}}
\newcommand*{\narrowsTo}[2][]{\starred{\narrows[#1]{#2}}}
\newcommand*{\narrowStep}[3][\genrule{l}{r}]{\narrows[{#1}]{\extraArg{#2}{#3}}}
\newcommand*{\nnarrows}{\not\leadsto}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        %
%   SEMANTICS INTERPRETATION FUNCTIONS   %
%                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% private (just for redefinition)
\newcommand*{\mathC}{\mathcal}
\newcommand*{\BehaSym}{\mathC{B}}
\newcommand*{\SemSym}{\mathC{S}}
\newcommand*{\TrSym}{\mathC{N}}
\newcommand*{\OsemSym}{\mathC{O}}
\newcommand*{\FSym}{\mathC{F}}
\newcommand*{\TpSym}{\mathC{P}}
\newcommand*{\evalSym}{\mathC{E}}
% public

\newcommand*{\Q}[2]{#1 \mathbin{\scriptstyle{\mathit{in}}} #2} % _ in _
\newcommand*{\Beha}[2][ss]{\syntaxoper{\BehaSym^{\mathit{#1}}}{#2}{}} %% general behavior macro
\newcommand*{\Sem}[2][\alpha]{\syntaxoper{\SemSym^{#1}}{#2}{}} % a semantics S
\newcommand*{\Tr}[3][]{\syntaxoperEXT{#2}{\TrSym_{#1}}{\Q{#2}{#3}}{}} %% semantics tree in P
% \newcommand*{\CA}[1]{\syntaxoper{\mathcal{CA}}{#1}{}} %% computed answers
% \newcommand*{\CAin}[2]{\CA{\Q{#1}{#2}}} %% computed answers in P

\newcommand*{\Osem}[1]{\syntaxoper{\OsemSym}{#1}{}} %% oper lfp characterization
\newcommand*{\F}[2][\alpha]{\syntaxoper{\FSym^{#1}}{#2}{}} %% general lfp macro
\newcommand*{\Tp}[3][\alpha]{\syntaxoper{\TpSym^{#1}}{#2}{{#3}}} %% general fixed-point op macro
\newcommand*{\TpN}[3][\alpha]{\iter{\Tp[{#1}]{#2}{}}{#3}} %% n-th iteration of the lfp conctruction
\newcommand*{\eval}[4][\alpha]{\syntaxoperEXT{#3}{\evalSym^{#1}}{\termres{#3}{#2}}{#4}}
\newcommand*{\evalrules}[3][\alpha]{\syntaxoper{\xi^{#1}}{#2}{#3}}
\newcommand*{\FUNeq}{\cong} %% variance on tree

\newcommand*{\I}[1][\alpha]{\Isym{#1}} %% generic interpretation
\newcommand*{\Sz}[1][\alpha]{\Ssym{#1}} %% generic specification
\newcommand*{\Rz}[1][\alpha]{\Rsym{#1}}
\newcommand*{\Isym}[1]{\mathC{I}^{#1}}
\newcommand*{\Ssym}[1]{\mathC{S}^{#1}}
\newcommand*{\Rsym}[1]{\mathC{X}^{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                          %
%   PROGRAM EQUIVALENCES   %
%                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\ProgEquiv}[3][]{#2 \thickapprox_{#1} #3} % program equivalence
\newcommand*{\BehaEq}[1][ss]{\ProgEquiv[\mathit{#1}]}
\newcommand*{\SemEq}[1][{\F[]{}}]{\ProgEquiv[{#1}]} %% program small-step operational equivalence


%%%%%%%%%%%%%%%%%%%
%                 %
%   PROOF TREES   %
%                 %
%%%%%%%%%%%%%%%%%%%

\newcommand{\ands}{\fbox{this should not be used, is just to prevent 
    unobserved redefinition of command \string\ands}}
\newcommand*{\sequent}[4][]{\gdef\and{\quad\hfill}
    \gdef\ands{\;\hfill\ldots\hfill\;}\global\setlabel{#1}
    {#1}\frac{\:\:#2\:\:}{\;#3\;}\;\text{\small%
\begin{tabular}{@{}l@{}} #4 \end{tabular}}}
    
\newcommand*{\twsequent}[3][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \and #3}}

\newcommand*{\thsequent}[4][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \and #3 \and #4}}

\newcommand*{\manysequent}[3][]{\Fbox{OBSOLETE}\sequent[{#1}]{#2 \ands #3}}

%%%%%%%%%%%%%
%           %
%   TREES   %
%           %
%%%%%%%%%%%%%

\DeclarePairedDelimiter{\Theight}{|}{|}
\newcommand*{\Tnode}[2]{\Fbox{$\llparenthesis\, #1 ; #2 \,\rrparenthesis$}} %% node constructor
\newcommand*{\Tpaths}{\parensmathoper{paths}}
\newcommand*{\Tmaxpaths}{\parensmathoper{maxpaths}}
\newcommand*{\Troot}{\parensmathoper{rt}} %% root node of a tree
\newcommand*{\Tsiblings}{\parensmathoper{siblings}}
\newcommand*{\Tsons}{\parensmathoper{sons}}
\newcommand*{\Tsteps}{\parensmathoper{steps}} %% steps set of a tree
\newcommand*{\Tstep}[4]{\quadruple{#1}{#2}{#3}{#4}} %% a relaxed-step in a tree
\newcommand*{\Tsubterm}[2]{\left. #1 \right\Downarrow_{#2}} %% induced subterm tree


%%%%%%%%%%%%%%%%%%%%%
%                   %
%   Miscellaneous   %
%                   %
%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\glb}{\ensuremath{\mathit{glb}}}
\newcommand*{\lub}{\ensuremath{\mathit{lub}}}
\newcommand*{\mgu}{\parensmathoper{mgu}} %% most general unifier

\newcommand*{\lfp}[1][]{\lfpof[{#1}]{}}
\newcommand*{\gfp}[1][]{\gfpof[{#1}]{}}
\newcommand*{\lfpof}[2][]{\mathoper{lfp}_{#1}\Braces{#2}}
\newcommand*{\gfpof}[2][]{\mathoper{gfp}_{#1}\Braces{#2}}

\newcommand*{\downiter}[2]{#1 \mathord{\downarrow} #2} %% iteration macro
\newcommand*{\equivClass}[2]{{#1}\big/_{\! #2}}
\newcommand*{\iter}[2]{#1 \mathord{\uparrow} #2} %% iteration macro
\newcommand*{\sameof}[3]{#1 \mapsto \iter{#2}{#3} (\mathit{#1})}


\newcommand*{\len}{\parensmathoper{length}}
\newcommand*{\prefixtree}{\parensmathoper{prfxtree}}


% COMPATIBILITY

% \newcommand*{\restriction}{\upharpoonright}

\backcompatibility{\rewrule}{\genrule}
\newcommand*{\rew}[2][noOpt]{\Fbox{USE \texttt{\string\rewrites}}\Fbox{$#1$}\rewrites[{#2}]}
\newcommand*{\rews}[2][noOpt]{\Fbox{USE \texttt{\string\rewritesTo}}\Fbox{$#1$}\rewritesTo[{#2}]}
\backcompatibility{\nrew}{\nrewrites}

\backcompatibility{\Subst}{\Substs}
\backcompatibility{\CSubst}{\CSubsts}
\backcompatibility{\Symbols}{\Fsyms}
\backcompatibility{\emptypos}{\rootPos}

%backward compatibility
\backcompatibility{\interp}{\interpC}
\backcompatibility{\leqI}{\leqIc}
\backcompatibility{\nleqI}{\nleqIc}


==> wgmacros-support.tex <==
% internals 

\providecommand*{\wgmWarn}[1]{\typeout{*** using WgMacros def of \string#1}}
\providecommand*{\ProvideWarnCommand}[2]{\providecommand*{#1}{\wgmWarn{#1}#2}}

\providecommand*{\backcompatibility}[2]{
  \newcommand*{#1}{\Fbox{USE \texttt{\string#2}}#2}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      %
%   Support (General Purpose) Macros   %
%                                      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\parensmathoper}[2]{\ensuremath{\mathoper{#1}\ifempty{#2}{}{(#2)}}}
\providecommand*{\syntaxoper}[3]{\mathoper{#1}\BBrackets[#3]{#2}}
\providecommand*{\syntaxoperEXT}[4]{\mathoper{#2}\ifempty{#1}{}{\llbracket#3\rrbracket_{#4}}}%

\providecommand*{\BBrackets}[2][]{\ifempty{#2}{}{\llbracket#2\rrbracket_{#1}}}
\providecommand*{\Braces}[2][]{\ifempty{#2}{}{( #2 )_{#1}}}%\big\big
\providecommand*{\extraArg}[2]{\ifempty{#1}{#2}{\ifempty{#2}{#1}{#1 ,\, #2}}}
\providecommand*{\extraArgSc}[2]{\ifempty{#2}{#1}{\ifempty{#1}{#2}{#1 ;\, #2}}}

\providecommand*{\monobioperator}[3]{
  \newcommand*{#1}[2]{{\ifempty{##2}{#3##1}{##1#2##2}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                            %
%   Support Macros defined by theorems.sty   %
%                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand*{\newsmartprefix}[2]{\wgmWarn{\newsmartprefix}}
\providecommand*{\newsmartsprefix}[2]{\wgmWarn{\newsmartsprefix}}
\providecommand*{\newdefinition}[1]{\wgmWarn{\newdefinition}\newdefinitionaux}
\providecommand*{\newdefinitionaux}[2][]{}
